Monitoring Algorithmic Fairness

Machine-learned systems are in widespread use for making decisions about humans, and it is important that they are fair, i.e., not biased against individuals based on sensitive attributes. We present runtime verification of algorithmic fairness for systems whose models are unknown, but are assumed to have a Markov chain structure. We introduce a specification language that can model many common algorithmic fairness properties, such as demographic parity, equal opportunity, and social burden. We build monitors that observe a long sequence of events as generated by a given system, and output, after each observation, a quantitative estimate of how fair or biased the system was on that run until that point in time. The estimate is proven to be correct modulo a variable error bound and a given confidence level, where the error bound gets tighter as the observed sequence gets longer. Our monitors are of two types, and use, respectively, frequentist and Bayesian statistical inference techniques. While the frequentist monitors compute estimates that are objectively correct with respect to the ground truth, the Bayesian monitors compute estimates that are correct subject to a given prior belief about the system's model. Using a prototype implementation, we show how we can monitor if a bank is fair in giving loans to applicants from different social backgrounds, and if a college is fair in admitting students while maintaining a reasonable financial burden on the society. Although they exhibit different theoretical complexities in certain cases, in our experiments, both frequentist and Bayesian monitors took less than a millisecond to update their verdicts after each observation.

==> frequentist_monitor_illustration.tex <==
% !TEX root=main.tex
\definecolor{Gray}{gray}{0.5}
%\definecolor{Blue}{blue}{0.5}
\colorlet{MyBlue}{blue!25!white}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.5pt] (char) {#1};}}
\newcommand*\myboxed[1]{\tikz[baseline=(char.base)]{
            \node[shape=rectangle,draw,inner sep=1pt] (char) {#1};}}
\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut
\begin{figure}
\centering
\tiny
\begin{tikzpicture}[scale=0.5,node distance=1.3cm]
	\node[draw,label=A]	(a)	at	(0,0)	{\begin{tabular}{ll}
%								\multicolumn{2}{c}{$p_Sp_Np_D$}\\
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$\bot$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=B]	(b)	[right of=a]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$2$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=C]	(c)	[right of=b]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $1$\\
								\rowcolor{MyBlue}
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$3$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=D]	(d)	[right of=c]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$2$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=E]	(e)	[right of=d]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								\rowcolor{MyBlue}
								$c_{24}$	& $1$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$4$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
							
	\node[draw,label=F]	(f)	[right of= e]{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $1$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$1$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=G]	(g)	[right of=f]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$c_1$	& $1$\\
								\rowcolor{MyBlue}
								$c_{12}$ & $1$ \\
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $1$\\
%								\rowfont{\color{Gray}}
								$x_1$	& $\emptyset$\\
%								\rowfont{\color{Gray}}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=H]	(h)	[right of=g]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$c_1$	& $0$\\
								\rowcolor{MyBlue}
								$c_{12}$ & $0$ \\
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $1$\\
								\rowcolor{MyBlue}
								$x_1$	& $2$\\
%								\rowfont{\color{Gray}}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label={[xshift=-0.2cm]I}]	(i)	[below =3cm of $(d.east) ! 0.5 !(e.west)$]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$1\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $1$\\
								$x_1$	& $2$\\
%								\rowfont{\color{Gray}}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=J]	(j)	[left of=i]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$1\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $1$\\
								\rowcolor{MyBlue}
								$c_{23}$	& $0$\\
								$c_{24}$	& $1$\\
								$x_1$	& $2$\\
								\rowcolor{MyBlue}
								$x_2$	& $3$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=K]	(k)	[left of=j]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$11\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $1$\\
								$x_1$	& $2$\\
								$x_2$	& $3$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=L]	(l)	[left of=k]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$11\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								\rowcolor{MyBlue}
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								\rowcolor{MyBlue}
								$x_2$	& $\circled{3}\myboxed{4}$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=M]	(m)	[above left=-1cm and 1cm of l]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$111$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								$x_2$	& $\circled{3}\myboxed{4}$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
								\rowcolor{MyBlue}
								$b$ &	$1$\\
								\rowcolor{MyBlue}
								$n$ &	$1$\\
								\rowcolor{MyBlue}
								$\verdict$	&	$[2\pm ?]$
							\end{tabular}};
	\node[draw,label=N]	(n)	[left=0.3cm of m]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								\rowcolor{MyBlue}
								$x_1$	& $\emptyset$\\
								\rowcolor{MyBlue}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
								\rowcolor{MyBlue}
								$b$ &	$0$\\
								$n$ &	$1$\\
								$\verdict$	&	$[2\pm ?]$
							\end{tabular}};
	\node[draw,label=O]	(o)	[below left=-1cm and 1cm of l]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$111$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								$x_2$	& $\circled{3}\myboxed{4}$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
								\rowcolor{MyBlue}
								$b$ &	$1$\\
								\rowcolor{MyBlue}
								$n$ &	$1$\\
								\rowcolor{MyBlue}
								$\verdict$	&	$[2\pm ?]$
							\end{tabular}};
	\node[draw,label=P]	(p)	[left=0.3cm of o]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								\rowcolor{MyBlue}
								$x_1$	& $\emptyset$\\
								\rowcolor{MyBlue}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
								\rowcolor{MyBlue}
								$b$ &	$0$\\
								$n$ &	$1$\\
								$\verdict$	&	$[2\pm ?]$
							\end{tabular}};
	\node[draw,label=Q]	(q)	[right of= i]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$1\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								\rowcolor{MyBlue}
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								\rowcolor{MyBlue}
								$x_2$	& $4$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=R]	(r)	[right of= q]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$10\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								$x_2$	& $4$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=S]	(s)	[right =0.4cm of r]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$100$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								$x_2$	& $4$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
								\rowcolor{MyBlue}
								$n$ &	$1$\\
								\rowcolor{MyBlue}
								$\verdict$	&	$[1\pm ?]$
							\end{tabular}};
	\node[draw,label=T]	(t)	[right=0.3cm of s]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								\rowcolor{MyBlue}
								$x_1$	& $\emptyset$\\
								\rowcolor{MyBlue}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
								$b$ &	$0$\\
								$n$ &	$1$\\
								$\verdict$	&	$[1\pm ?]$
							\end{tabular}};
							
%	\path[->,draw]	(a)	--	(b)
%					(b)	--	(c)
%					(c)	--	(d)
%					(d)	--	(e)
%					(e)	--	(f)
%					(f)	--	(g)
%					(g)	--	(h);
	\draw[->]	(a)	-- node[above]	{$2$}	(b);
	\draw[->]	(b)	-- node[above]	{$3$}	(c);
	\draw[->]	(c)	-- node[above]	{$2$}	(d);
	\draw[->]	(d)	-- node[above]	{$4$}	(e);
	\draw[->]	(e)	-- node[above]	{$1$}	(f);
	\draw[->]	(f)	-- node[above]	{$2$}	(g);
	\draw[->]	(g)	-- node[above]	{L\ref{alg:freq:next:g}}	(h);
	\draw[->] (h.south) |- ($(h.south) - (0,5mm)$) -| node[below right]	{L\ref{alg:freq:next:eval xiS}} (i.north);

	\draw[->]	(i)	-- node[above]	{L\ref{alg:freq:next:h}}	(j);
	\draw[->]	(j)	-- node[above]	{L\ref{alg:freq:next:eval xiN}}	(k);
	\draw[->]	(k)	-- 	(l);
	\draw[->]	(l)	-- node[right]	{L\ref{alg:freq:next:eval xiD}}	(m);
	\draw[->]	(m)	-- 	(n);
	
	\draw[->]	(l)	-- node[left]	{L\ref{alg:freq:next:eval xiD}}	(o);
	\draw[->]	(o)	--	(p);
	
	\draw[->]	(i)	-- node[above]	{L\ref{alg:freq:next:h}}	(q);
	\draw[->]	(q)	-- node[above]	{L\ref{alg:freq:next:eval xiN}}	(r);
	\draw[->]	(r)	-- node[above]	{L\ref{alg:freq:next:eval xiD}}	(s);
	\draw[->]	(s)	--	(t);
	
	\begin{scope}[on background layer]
	\draw[fill=Gray!15!white]	($(h.north)+(-1.2,0.1)$) -- ($(h.north)+(1,0.1)$) -- ($(s.south)+(1.5,-1)$) -- ($(o.south)+(-1.5,-1)$) -- ($(m.north)+(-1.5,0.5)$) -- ($(m.north)+(1.5,0.5)$) -- ($(m.north)+(1.5,-1.5)$) -- ($(h.south)+(-1.2,-0.1)$) -- cycle;
	\end{scope}


\end{tikzpicture}
\caption{A path of the monitor for the property $\varphi = v_{12}+v_{23}\div (v_{12}+v_{24})$ on the word $232412$.
The top row of every node represents the state of the monitor, specified using the vector $(p_S,p_N,p_D)$, while the rest of the node captures the values of the counters/registers.
Transitions are triggered either externally through arrival of a new symbol or internally (the grey region) as part of the algorithm.
%The nodes in the grey region represent one execution of the $\mathit{Next}()$ function, that comprises of a sequence of state transitions.
The labels on the transitions represent the respective new symbol or the respective line number in the $\mathit{Next}()$ function.
The circle and the square markers in nodes L, M, and O represent the index of $x_2$ that $t_{23}$ and $t_{24}$ point at.
\todo{Calculate the bounds using Chebyshev's inequality in M, O, S. Make the grey box nicer.}}
\label{fig:example run of frequentist monitor}
\end{figure}

==> frequentist_monitor_illustration_division_free.tex <==
% !TEX root=main.tex
\definecolor{Gray}{gray}{0.5}
%\definecolor{Blue}{blue}{0.5}
\colorlet{MyBlue}{blue!25!white}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.5pt] (char) {#1};}}
\newcommand*\myboxed[1]{\tikz[baseline=(char.base)]{
            \node[shape=rectangle,draw,inner sep=1pt] (char) {#1};}}
\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut
\begin{figure}
\centering
\tiny
\begin{tikzpicture}[scale=0.5,node distance=1.3cm]
	\node[draw,label=A]	(a)	at	(0,0)	{\begin{tabular}{ll}
%								\multicolumn{2}{c}{$p_Sp_Np_D$}\\
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$\bot$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=B]	(b)	[right of=a]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$2$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=C]	(c)	[right of=b]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $1$\\
								\rowcolor{MyBlue}
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$3$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=D]	(d)	[right of=c]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$2$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=E]	(e)	[right of=d]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								\rowcolor{MyBlue}
								$c_{24}$	& $1$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$4$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
							
	\node[draw,label=F]	(f)	[right of= e]{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $1$\\
								$x_1$	& $\emptyset$\\
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$1$\\
								$b$ &	$0$\\
								$n$ &	$0$\\
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=G]	(g)	[right of=f]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$c_1$	& $1$\\
								\rowcolor{MyBlue}
								$c_{12}$ & $1$ \\
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $1$\\
%								\rowfont{\color{Gray}}
								$x_1$	& $\emptyset$\\
%								\rowfont{\color{Gray}}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=H]	(h)	[right of=g]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								\rowcolor{MyBlue}
								$c_1$	& $0$\\
								\rowcolor{MyBlue}
								$c_{12}$ & $0$ \\
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $1$\\
								\rowcolor{MyBlue}
								$x_1$	& $2$\\
%								\rowfont{\color{Gray}}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label={[xshift=-0.2cm]I}]	(i)	[below =3cm of $(d.east) ! 0.5 !(e.west)$]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$1\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $2$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $1$\\
								$x_1$	& $2$\\
%								\rowfont{\color{Gray}}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=J]	(j)	[left of=i]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$1\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $1$\\
								\rowcolor{MyBlue}
								$c_{23}$	& $0$\\
								$c_{24}$	& $1$\\
								$x_1$	& $2$\\
								\rowcolor{MyBlue}
								$x_2$	& $3$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=K]	(k)	[left of=j]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$11\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $1$\\
								$x_1$	& $2$\\
								$x_2$	& $3$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=L]	(l)	[left of=k]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$11\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								\rowcolor{MyBlue}
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								\rowcolor{MyBlue}
								$x_2$	& $\circled{3}\myboxed{4}$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=M]	(m)	[left=0.5cm of l]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$111$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								$x_2$	& $\circled{3}\myboxed{4}$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
								\rowcolor{MyBlue}
								$b$ &	$1$\\
								\rowcolor{MyBlue}
								$n$ &	$1$\\
								\rowcolor{MyBlue}
								$\verdict$	&	$[2\pm 4.1]$
							\end{tabular}};
	\node[draw,label=N]	(n)	[left=0.3cm of m]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $0$\\
								$c_{23}$	& $0$\\
								$c_{24}$	& $0$\\
								\rowcolor{MyBlue}
								$x_1$	& $\emptyset$\\
								\rowcolor{MyBlue}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
								\rowcolor{MyBlue}
								$b$ &	$0$\\
								$n$ &	$1$\\
								$\verdict$	&	$[2\pm 4.1]$
							\end{tabular}};
%	\node[draw,label=O]	(o)	[below left=-1cm and 1cm of l]	{\begin{tabular}{ll}
%								\rowcolor{MyBlue}
%								\multicolumn{2}{c}{$111$}\\
%								\hline\\[-2.5ex]
%								$c_1$	& $0$\\
%								$c_{12}$ & $0$ \\
%								$c_2$	& $0$\\
%								$c_{23}$	& $0$\\
%								$c_{24}$	& $0$\\
%								$x_1$	& $2$\\
%								$x_2$	& $\circled{3}\myboxed{4}$\\
%								\hline\\[-2.5ex]
%								$\sigma'$ &	$2$\\
%								\rowcolor{MyBlue}
%								$b$ &	$1$\\
%								\rowcolor{MyBlue}
%								$n$ &	$1$\\
%								\rowcolor{MyBlue}
%								$\verdict$	&	$[2\pm ?]$
%							\end{tabular}};
%	\node[draw,label=P]	(p)	[left=0.3cm of o]	{\begin{tabular}{ll}
%								\multicolumn{2}{c}{$\bot\bot\bot$}\\
%								\hline\\[-2.5ex]
%								$c_1$	& $0$\\
%								$c_{12}$ & $0$ \\
%								$c_2$	& $0$\\
%								$c_{23}$	& $0$\\
%								$c_{24}$	& $0$\\
%								\rowcolor{MyBlue}
%								$x_1$	& $\emptyset$\\
%								\rowcolor{MyBlue}
%								$x_2$	& $\emptyset$\\
%								\hline\\[-2.5ex]
%								$\sigma'$ &	$2$\\
%								\rowcolor{MyBlue}
%								$b$ &	$0$\\
%								$n$ &	$1$\\
%								$\verdict$	&	$[2\pm ?]$
%							\end{tabular}};
	\node[draw,label=Q]	(q)	[right of= i]	{\begin{tabular}{ll}
								\multicolumn{2}{c}{$1\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								\rowcolor{MyBlue}
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								\rowcolor{MyBlue}
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								\rowcolor{MyBlue}
								$x_2$	& $4$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=R]	(r)	[right of= q]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$10\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								$x_2$	& $4$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
%								\rowfont{\color{Gray}}
								$n$ &	$0$\\
%								\rowfont{\color{Gray}}
								$\verdict$	&	$\bot$
							\end{tabular}};
	\node[draw,label=S]	(s)	[right =0.4cm of r]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$100$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								$x_1$	& $2$\\
								$x_2$	& $4$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
%								\rowfont{\color{Gray}}
								$b$ &	$0$\\
								\rowcolor{MyBlue}
								$n$ &	$1$\\
								\rowcolor{MyBlue}
								$\verdict$	&	$[1\pm 4.1]$
							\end{tabular}};
	\node[draw,label=T]	(t)	[right=0.3cm of s]	{\begin{tabular}{ll}
								\rowcolor{MyBlue}
								\multicolumn{2}{c}{$\bot\bot\bot$}\\
								\hline\\[-2.5ex]
								$c_1$	& $0$\\
								$c_{12}$ & $0$ \\
								$c_2$	& $1$\\
								$c_{23}$	& $1$\\
								$c_{24}$	& $0$\\
								\rowcolor{MyBlue}
								$x_1$	& $\emptyset$\\
								\rowcolor{MyBlue}
								$x_2$	& $\emptyset$\\
								\hline\\[-2.5ex]
								$\sigma'$ &	$2$\\
								$b$ &	$0$\\
								$n$ &	$1$\\
								$\verdict$	&	$[1\pm 4.1]$
							\end{tabular}};
							
%	\path[->,draw]	(a)	--	(b)
%					(b)	--	(c)
%					(c)	--	(d)
%					(d)	--	(e)
%					(e)	--	(f)
%					(f)	--	(g)
%					(g)	--	(h);
	\draw[->]	(a)	-- node[above]	{$2$}	(b);
	\draw[->]	(b)	-- node[above]	{$3$}	(c);
	\draw[->]	(c)	-- node[above]	{$2$}	(d);
	\draw[->]	(d)	-- node[above]	{$4$}	(e);
	\draw[->]	(e)	-- node[above]	{$1$}	(f);
	\draw[->]	(f)	-- node[above]	{$2$}	(g);
	\draw[->]	(g)	-- node[above]	{L\ref{alg:freq:next:g}}	(h);
	\draw[->] (h.south) |- ($(h.south) - (0,5mm)$) -| node[below right]	{L\ref{alg:freq:next:eval xiS}} (i.north);

	\draw[->]	(i)	-- node[above]	{L\ref{alg:freq:next:h}}	(j);
	\draw[->]	(j)	-- node[above]	{L\ref{alg:freq:next:eval xiN}}	(k);
	\draw[->]	(k)	-- 	(l);
	\draw[->]	(l)	-- node[above]	{L\ref{alg:freq:next:eval xiD}}	(m);
	\draw[->]	(m)	-- 	(n);
	
%	\draw[->]	(l)	-- node[left]	{L\ref{alg:freq:next:eval xiD}}	(o);
%	\draw[->]	(o)	--	(p);
	
	\draw[->]	(i)	-- node[above]	{L\ref{alg:freq:next:h}}	(q);
	\draw[->]	(q)	-- node[above]	{L\ref{alg:freq:next:eval xiN}}	(r);
	\draw[->]	(r)	-- node[above]	{L\ref{alg:freq:next:eval xiD}}	(s);
	\draw[->]	(s)	--	(t);
	
	\begin{scope}[on background layer]
	\draw[fill=Gray!15!white]	($(h.north)+(-1.2,0.1)$) -- ($(h.north)+(1,0.1)$) -- ($(s.south)+(1.5,-1)$) -- ($(m.south)+(-1.5,-1)$) -- ($(m.north)+(-1.5,0.5)$) -- ($(m.north)+(1.5,0.5)$) --  ($(h.south)+(-1.2,-0.1)$) -- cycle;
	\end{scope}


\end{tikzpicture}
\caption{A path of the monitor for the property $\varphi = v_{12}+v_{23}* (v_{12}+v_{24})$ on the word $232412$.
The top row of every node shows an intermediate evaluation of the variables $(v_{12},v_{23},(v_{12}+v_{24}))$, while the rest of every node captures the values of the counters/registers.
%Every node displays the snapshot of the values of the counters/registers.
Transitions are triggered either externally through arrival of a new symbol or internally (the grey region) as part of the algorithm.
%The nodes in the grey region represent one execution of the $\mathit{Next}()$ function, that comprises of a sequence of state transitions.
The labels on the transitions represent the respective new symbol or the respective line number in the $\mathit{Next}()$ function.
The circle and the square markers in nodes L, M, and O represent the index of $x_2$ that $t_{23}$ and $t_{24}$ point at.
After consuming the given run $232412$, the monitor arrives at the states $N$ and $T$ with equal probability, which output the $95\%$ confidence intervals $[2\pm 4.1]$ and $[1\pm 4.1]$ respectively.
\todo{Make the figure fit in the boundary, make the grey box nicer.}}
\label{fig:example run of frequentist monitor}
\end{figure}
